Correspondence Matrices are Underrated

Point-cloud registration (PCR) is an important task in various applications such as robotic manipulation, augmented and virtual reality, SLAM, etc. PCR is an optimization problem involving minimization over two different types of interdependent variables: transformation parameters and point-to-point correspondences. Recent developments in deep-learning have produced computationally fast approaches for PCR. The loss functions that are optimized in these networks are based on the error in the transformation parameters. We hypothesize that these methods would perform significantly better if they calculated their loss function using correspondence error instead of only using error in transformation parameters. We define correspondence error as a metric based on incorrectly matched point pairs. We provide a fundamental explanation for why this is the case and test our hypothesis by modifying existing methods to use correspondence-based loss instead of transformation-based loss. These experiments show that the modified networks converge faster and register more accurately even at larger misalignment when compared to the original networks.

==> rahul_suggestions.tex <==
{\bf Experiment Suggestions}

{\bf ModelNet 40}
\begin{itemize}
    \item ModelNet40: Compare with RPM-Net, RPM, DCP\_v2, PointNetLK, PCRNet, PRNet, FGR, ICP, RANSAC. No need to implement methods designed for 3dMatch.
    \item ModelNet40: RPM-Net has conducted 3 experiments and results of all other models are readily available. 1) clean data (identical), 2) gaussian noise (nonidentical+jittered), 3) partial-to-full (nonidentical+jittered).
    \item ModelNet40: If our outlier filtering mechanism works, we can conduct 1 more experiment on M40: 1) partial-to-partial.
    \item ModelNet40: Another good experiment can be comparing the training on whole correspondence matrix (like ours) vs training only on src src\_corr pairs (like done in MVR and DGR). But other experiment settings including feature descriptor can be kept same.
\end{itemize}

{\bf Stanford 3D Repository}

Another good dataset.


{\bf Theoretical Argument}

Many of the recent networks are designed to estimate the correspondence matrix which will minimize the transformation loss.

Consider an optimization problem with transformation loss as objective and correspondence matrix as parameters.

T* = argmin[T(X) - YC]

X and Y are the constants for a point cloud, hence 

T* = f(C)

This is a non convex function with multiple local minima and global minima (need a proof! or example)

As DCP searches the C space in an unconstrained fashion, it has the probability to get stuck in local minima. We constrain the network to predict C values close to a C* value where we know that C* is one such point of global minima. We thus reduce the search space leading to a faster convergence.

DCP tries to solve a non convex optimization problem.

On the other hand, estimating C* from C (using cross entropy) is a convex problem thus a single global minima.

(Though training network weights is non convex but atleast has a single global minima)

==> tejas_points.tex <==

\begin{itemize}
    \item Correspondences are important
    \item Deep learning methods take in pointclouds and output transformations. Empirically we show that instead it should predict correspondences cause small corruption in transformation leads to large rotation error!
    \item List out methods DCP, PointnetLK, PCRNet, PRNet and there working. 
    \item DGR, MVR work better cause work on correspondeces 
    \item We can write as not a new method but a method to tell why is it good to train on correspondences.    
    \item Results of \% corrupt correspondence matrix  and show rotation error
    corrupt rotation matrix  and show rotation error
    \item Paper summary in intro.
    \item Define what do you mean by global registration. Contribution: 1. Empirically show Why should you train on correspondences. 2. We are also giving a method which can deal with partial global registration as a virtue of training on correpondences. Potentailly outliers too? 
    \item Reverse engineer on the contribution to modify introduction.
    \item Write abstract in parallel.
    \item Comparison with FCGF?
    \item One step outlier removal?
    \item Graph of initial misalignment vs error 

    
\end{itemize}

